Pessimistic Model-based Offline Reinforcement Learning under Partial Coverage

We study model-based offline Reinforcement Learning with general function approximation without a full coverage assumption on the offline data distribution. We present an algorithm named Constrained Pessimistic Policy Optimization (CPPO)which leverages a general function class and uses a constraint over the model class to encode pessimism. Under the assumption that the ground truth model belongs to our function class (i.e., realizability in the function class), CPPO has a PAC guarantee with offline data only providing partial coverage, i.e., it can learn a policy that competes against any policy that is covered by the offline data. We then demonstrate that this algorithmic framework can be applied to many specialized Markov Decision Processes where additional structural assumptions can further refine the concept of partial coverage. Two notable examples are: (1) low-rank MDP with representation learning where the partial coverage condition is defined using a relative condition number measured by the unknown ground truth feature representation; (2) factored MDP where the partial coverage condition is defined using density ratio based concentrability coefficients associated with individual factors.

==> add.tex <==

\subsection{Another algorithm}

Consider the following algorithm: 
\begin{align*}
    &\min_{w_h}w^{\top}_0\phi(s_0,\pi), \|w_h\|^2_2\leq  W,\EE_{\Dcal}[\{w^{\top}_{h}\phi(s_h,a_h)+r_h- w^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2]\leq \epsilon+\epsilon' \\
    &\epsilon' =\sqrt{c(d+\log|\Pi|+\log(1/\delta))/n} \\ 
   & \epsilon= W\{d+\log(|\Pi|/\delta)\}/n.  
\end{align*}
Here, $\Dcal$ is the trajectory offline data following the policy $\pi_b$. 
Then, the bound is 
\begin{align*}
   V^{\pi}-V^{\hat \pi}\leq \sum_t \sqrt{C_{\pi,t}( \epsilon+ \epsilon') }.
\end{align*}
where $C_{\pi,t}$ is the relative condition number. Note when we use the linear greedy policy class, $\log |\Pi|\approx d$. 
\begin{proof}
~
\paragraph{Feasibility}
LSTD satisfies the equation: 
\begin{align*}
    \EE_{\Dcal}[\{w^{\top}_{h}\phi(s_h,a_h)+r_h- w^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2]=0.  
\end{align*}
Thus, the constrain set is feasible. 

\paragraph{Pessimism}

We show the true ${w^{\star}}_h$ is included in the ball. 
\begin{align*}
    & \EE_{\Dcal}[\{{w^{\star}}^{\top}_{h}\phi(s_h,a_h)+r_h- {w^{\star}}^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2]\\
    &= \EE_{\Dcal}[\{{w^{\star}}^{\top}_{h}\phi(s_h,a_h)+r_h- {w^{\star}}^{\top}_{h+1}M_{\pi}\phi(s_h,a_h)\}^2 ]+W \EE_{\Dcal}[\|\{\hat M_{\pi}-M_{\pi}\}\phi(s_h,a_h)\|^2_2]\\
      &=%
       W\EE_{\Dcal}[\beta'^2\| \phi(s_h,a_h)\|^2_{\Sigma^{-1}_{n,h}}]\leq \epsilon,\quad \epsilon \coloneqq W\{d+\log(1/\delta)\}/n. 
\end{align*}
Recall $\beta'=\sqrt{\{d+\log(|\Pi|/\delta)\}} $. (We need union bound for $\pi\in \Pi$ here). 



\paragraph{Show the solution is closed to the true policy value}

\begin{align*}
    | V^{\pi}-\hat V^{\pi}|&=|\sum_{t=0}^{H-1} \EE_{(s,a)\sim d^{\pi}_{P^{\star},t}}[\Bcal \hat Q_{t+1}(s,a)-\hat Q_t(s,a)] |\tag{Telescoping sum} \\
    & =| \sum_{t=0}^{H-1} \EE_{(s,a)\sim d^{\pi}_{P^{\star},t}}[r(s,a)+ \hat w^{\top}_{t+1}M_{\pi}\phi(s,a)-\hat w^{\top}_t\phi(s,a) ]|\\
     & \leq  \sum_{t=0}^{H-1} \sqrt{\EE_{(s,a)\sim d^{\pi}_{P^{\star},t}}[|r(s,a)+ \hat w^{\top}_{t+1}M_{\pi}\phi(s,a)-\hat w^{\top}_t\phi(s,a) |^2]}\\ 
        & \leq  \sum_{t=0}^{H-1} \sqrt{C_{\pi_b,t}\EE_{(s,a)\sim  d^{\pi_b}_{P^{\star},t}}|r(s,a)+ \hat w^{\top}_{t+1}M_{\pi}\phi(s,a)-\hat w^{\top}_t\phi(s,a) |^2]}\\ 
\end{align*}   


Here,
\begin{align*}
    & \EE_{\Dcal}[\{\hat w^{\top}_{h}\phi(s_h,a_h)+r_h- \hat w^{\top}_{h+1}M_{\pi}\phi(s_h,a_h)\}^2]\\
    &= \EE_{\Dcal}[\{\hat w^{\top}_{h}\phi(s_h,a_h)+r_h- \hat w^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2+   W \EE_{\Dcal}[\|\{\hat M_{\pi}-M_{\pi}\}\phi(s_h,a_h)\|^2_2]\\
    &=\EE_{\Dcal}[\{\hat w^{\top}_{h}\phi(s_h,a_h)+r_h-\hat w^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2]+\epsilon \leq 2\epsilon+\epsilon' .  
\end{align*}

We would also use the following concentration inequality. From Hoeffeding inequality plus the union bound over $\|w\|_2\leq W$ and $\pi\in \Pi$, we have, for $\forall w$, $\forall \pi$, 
\begin{align}
    &|\EE_{\Dcal}[\{ w^{\top}_{h}\phi(s_h,a_h)+r_h- w^{\top}_{h+1}M_{\pi}\phi(s_h,a_h)\}^2]- \EE_{(s,a)\sim  d^{\pi_b}_{P^{\star},t}}[\{ w^{\top}_{h}\phi(s_h,a_h)+r_h-  w^{\top}_{h+1}M_{\pi}\phi(s_h,a_h)\}^2]
    | \leq \epsilon '\label{eq:union}\\
    & \epsilon '=H\sqrt{c\{d+\log|\Pi|+\log(1/\delta)\}/n}. \tag{$d$ comes from $\forall w\in W$. }
\end{align}

Finally, using \pref{eq:union}, we have 
\begin{align*}
  \EE_{(s,a)\sim  d^{\pi_b}_{P^{\star},t}}|r(s_t,a_t)+ \hat w^{\top}_{t+1}M_{\pi}\phi(s,a)-\hat w^{\top}_t\phi(s,a) |^2 \leq 2\epsilon+2\epsilon'. 
\end{align*}

Thus, 
\begin{align*}
    | V^{\pi}-\hat V^{\pi}|\leq 2\epsilon+2\epsilon'. 
\end{align*}

\end{proof}


\section{Optimistic algorithm}


Consider the following algorithm: 
\begin{align*}
   \pi^m= &\max_{\pi}\max_{w_h}w^{\top}_0\phi(s_0,\pi), \|w_h\|_2\leq  W,\EE_{\Dcal_m}[\{w^{\top}_{h}\phi(s_h,a_h)+r_h- w^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2]\leq \epsilon. 
\end{align*}
($m$ is the index for episodes, $\Dcal_m$ is the collection of the data following $\pi^{m-1}$ to $\pi^1$ . 
More specifically, $\Dcal_m=\{s^i_h,a^i_h,r^i_h\}^{i=m-1,h=H-1}_{i=1,h=0}$. 

\begin{proof}
~
\paragraph{Optimism}
Need to check $w^{\star}_h$ (true $w_h$) satisfies the constraint. This is 
\begin{align*}
    &\EE_{\Dcal_m}[\{\{w^{\star}\}^{\top}_{h}\phi(s_h,a_h)+r_h- \{w^{\star}\}^{\top}_{h+1}\hat M_{\pi}\phi(s_h,a_h)\}^2]\\
   &\leq \EE_{\Dcal_m}[\{\{w^{\star}\}^{\top}_{h}\phi(s_h,a_h)+r_h- \{w^{\star}\}^{\top}_{h+1} M_{\pi}\phi(s_h,a_h)\}^2]+\EE_{\Dcal_m}[W\|(\hat M_{\pi}-M_{\pi})\phi(s,a)\|_2  ]\\
     &\leq \EE_{\Dcal_m}[W\|(\hat M_{\pi}-M_{\pi})\phi(s,a)\|_2  ]. 
\end{align*}
The second term is upper-bounded by
\begin{align*}
    &\EE_{(s,a) \sim \Dcal_m}[W\beta'\|\phi(s,a)\|_{\{\Sigma^{m}_h\}^{-1}}],\quad \Sigma^{m}_h=I+\sum_{i}^{m-1}\phi(s^i_h,a^i_h)\phi^{\top}(s^i_h,a^i_h)\\
    &\leq W\beta'/m. 
\end{align*}

Here, we have
\begin{align*}
      V^{\star}-V^{\pi_m}\leq \hat V^{\pi^{\star}}-V^{\pi_m}\leq \hat V^{\pi_m}-V^{\pi_m}.
\end{align*}

\paragraph{Regret}

\begin{align*}
\hat V^{\pi_m}-V^{\pi_m} &\leq \sum_h \EE_{(s,a)\sim d^{\pi_m}_h}[\hat Q^m_h(s,a)-\Tcal \hat Q^m_{t+1}(s,a)  ]\\
    &\leq \sum_h \EE_{(s,a)\sim d^{\pi_m}_h}[\hat w^{\top}_h \phi(s,a)-r(s,a)-\hat w^{\top}_{h+1} M_{\pi}\phi(s,a)]\\ 
       &\leq \sum_h \EE_{(s,a)\sim d^{\pi_m}_h}[\hat w^{\top}_h \phi(s,a)-r(s,a)-\hat w^{\top}_{h+1} \hat M_{\pi}\phi(s,a)]+\EE_{(s,a)\sim d^{\pi_m}_h}[W\|(\hat M_{\pi}-M_{\pi})\phi(s,a)\|_2  ]. 
\end{align*}
The second term is upper-bounded by
\begin{align*}
    \EE_{(s,a)\sim d^{\pi_m}_h}[W\beta'\|\phi(s,a)\|_{\Sigma^{-1,m}_h}],\quad \Sigma^{m}_h=I+\sum_{i}^{m-1}\phi(s^i_h,a^i_h)\phi^{\top}(s^i_h,a^i_h). 
\end{align*}
where $\beta'=\sqrt{d+\log(|\Pi|/\delta})$. This is handed by elliptical potential lemma. 
The first term is upper-bounded by  ?????
\masa{$d^{\pi_m}_h$ is not covered by $\Dcal_m$?}
\end{proof}


==> analysis.tex <==
\section{Analysis of PS-PO }
\label{sec:analysis}
We analyze PS-PO and establish its Bayesian suboptimality gap bound. Our analysis is a combination of the idea of pessimism and policy optimization bound of soft policy update. Notably, our algorithm does not explicitly uses pessimism reward penalty or version space, but our analysis will still rely on the idea of pessimism. To do that, we first analyze a na\"ive model-based posterior sampling algorithm to get an intuition of how the pessimism is \emph{automatically} induced. Then, we move onto the analysis of our proposed algorithm PS-PO. %


\subsection{The Implicit Pessimism in Posterior Sampling}

As a warm-up, we analyze the following na\"ive (single-shot) posterior sampling algorithm. This algorithm takes the model $P$ sampled from the posterior $\beta(\cdot\mid \Dcal)$ and outputs the optimal policy for this model $P$ (i.e., by using a planning oracle). Namely the algorithm has the following two steps: \wen{note that i removed the algorithm box and only list the algorithm in the equation below, I think we should not put too much effort on this one, this one should just be treated as a warm up..}
\begin{align*}
P\sim \beta(\cdot | \Dcal), \quad \pi(P) = \argmax_{\pi} V^{\pi}_{P}.
\end{align*}


To analyze the above two step algorithm in the Bayesian setting, we first introduce some additional notations. We first define a function over the policy class depending on $\Dcal$: $L(\pi;\Dcal):\Pi \to [0,H]$. %
Then, inspired by \citet{RussoDaniel2014LtOv}, for the model $P$ sampled from $\beta(\cdot | \Dcal)$, we have the following decomposition for Bayesian suboptimaligy gap:  \wen{notation: use the $\pi(P)$ notations below}
\begin{align*} 
\mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}   -  V^{\pi(P)}_{P^{\star}} \right] & =\mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}  -L(\pi(P^{\star});\Dcal)+ L(\pi(P^{\star});\Dcal)- V^{\pi(P)}_{P^{\star}} \right]\\ 
&=\mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}  -L(\pi(P^{\star});\Dcal)+ \EE[L(\pi(P^{\star});\Dcal)\mid \Dcal]- V^{\pi(P)}_{P^{\star}} \right]\\
&=\mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}  -L(\pi(P^{\star});\Dcal)+ L(\pi(P);\Dcal)- V^{\pi(P)}_{P^{\star}} \right]. 
\end{align*}
We use $\mathbb{E}\left[ L(\pi(P^{\star});\Dcal)  | \Dcal \right] = \mathbb{E}\left[  L(\pi(P);\Dcal)   | \Dcal\right]$ as $P$ and $P^\star$ are independently distributed from $\beta(\cdot | \Dcal)$. Then, given $P^\star$ with $\Dcal$ generated based on $P^\star$ (i.e., $s,a\sim \rho,s'\sim P^\star(\cdot | s,a)$), if $L(\pi;\Dcal)$ gives a lower confidence bound of $V^{\pi}_{P^\star}$, such that $\forall \pi \in \Pi: V^{\pi}_{P^{\star}}\geq L(\pi;\Dcal)$, we have 
\begin{align}\label{eq:pessimism}
    \mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}   -  V^{\pi(P)}_{P^{\star}} \right]\leq \mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}  -L(\pi(P^{\star});\Dcal)\right]. 
\end{align}
This is summarized into the following theorem. 
\begin{theorem}\label{thm:naive}
Given a model $P^{\star}$ on the support $\{P^{\star}:\beta(P^{\star})>0\}$ and an offline dataset $\Dcal$ generated based on $P^{\star}$, suppose we have $L(\pi;\Dcal):\Pi \to [0,H]$ s.t. with probability $1-\delta$,  $L(\pi;\Dcal)\leq V^{\pi}_{P^{\star}},\forall \pi \in \Pi$. Then,  we have 
\begin{align*}
        \mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}  -  V^{\pi(P)}_{P^{\star}} \right]\leq \mathbb{E}\left[  V^{\pi(P^{\star})}_{P^\star}  -L(\pi(P^{\star});\Dcal)\right]+2\delta H. 
\end{align*}
\end{theorem}

This result satisfies our desiderata, i.e., we can obtain the bound for Bayesian sumoptimality gap under the partial coverage as we only need to concern about the distribution $d^{\pi(P^{*})}_{P^{*}}$. In the Bayesian setting, the analogue of the density ratio and relative condition number are  \wen{if we always compare to the optimal policy of $P^\star$, then these concentrability coefficient should not depend on $\pi^\star$ anymore, as we take expectation over the prior already..}\masa{fixed} \wen{I changed the notations below using subscript $\beta$, please double check:}
\begin{align}\label{eq:Bayesian}
    C^{\text{Bayes}}_{\beta} & =\max_{(s,a)} \frac{\EE_{P^{*}\sim \beta}[d^{\pi(P^{*})}_{P^{*}}(s,a)]}{\rho(s,a)},\\
    \bar C^{\text{Bayes}}_{\beta}&=\sup_{x\in \RR^d}\frac{x^{\top}, \Sigma^{\text{Bayes}}_{\beta}x}{x^{\top}\Sigma_{\rho}x}\\
   \Sigma^{\text{Bayes}}_{\beta} &= EE_{P^{*}\sim \beta,(s,a)\sim d^{\pi(P^{*})}_{P^{*}}}[\phi(s,a)\phi(s,a)^{\top}],\quad     \Sigma_{\rho}=\EE_{\rho}[\phi(s,a)\phi(s,a)^{\top}],
\end{align} where $\phi$ is the known feature in KNR (we can replace $\phi$ in the above quantities by the unknown true feature $\phi^\star$ in the low-rank MDP setting). 
Comparing to the frequentist quantities, we consider the averaged version with respect to the prior $\beta$.  This depends on the comparator policy $\pi(P^{\star})$ but \emph{not} all policies in the policy class. The partial coverage means these type of quantities are upper-bounded by some constant. 

To obtain Bayesia suboptimality gap bounds from \pref{thm:naive} under the partial coverage, we need to design $L(\pi;\Dcal)$ on a case-by-case basis. The first choice is $\min_{M}V^{\pi}_{M\in \Mcal_{\Dcal}}$ in \pref{alg:main_version}, which satisfies the condition $\min_{M}V^{\pi}_{M\in \Mcal_{\Dcal}} \leq V^{\pi}_{P^{\star}},\forall \pi\in \Pi$.  %
Then, we can plug the frequentist optimality gap result \pref{thm:version} into \pref{thm:naive}, which leads to the Bayesian suboptimality gap result under partial coverage. Another choice is a bonus-type offline policy evaluation result \citep{ChangJonathanD2021MCSi}.  Given the dataset $\Dcal$, we compute a model estimator $\widehat{P}(\cdot | s,a)$ and a model uncertainty $\sigma(s,a)$ s.t.  $\forall s,a: \; \| \widehat{P}(\cdot | s,a) - P(\cdot|s,a) \|_{1} \leq \sigma(s,a)$, then we can design a reward penalty $b(s,a) = H\sigma(s,a)$ so that $V^{\pi}_{\widehat{P}, r - b}$ satisfies the condition  $V^{\pi}_{\widehat{P}, r - b}\leq V^{\pi}_{P^{\star}},\forall \pi\in \Pi$, where $V^{\pi}_{\widehat{P}, r - b}$ is a policy value under a transition $\widehat{P}$, a reward $r-b$ and a policy $\pi$. Then, by translating the frequentist result of \citet{ChangJonathanD2021MCSi} into the Bayesian setting, we can obtain the Bayesian suboptimality bound under the partial coverage. We will see more specific bounds in \pref{sec:example}. 

\begin{remark}
The above derivation of \pref{thm:naive} illustrates the difference between pessimism and optimism. Suppose $L$ is an optimistitc upper bound such that $\forall \pi \in \Pi: V^{\pi}_P\leq L(\pi;\Dcal). $
Then, 
\begin{align}\label{eq:optimisim}
    \mathbb{E}\left[  V^{\pi(P^{*})}_{P^*}   -  V^{\pi(P)}_{P^{*}} \right]\leq \mathbb{E}\left[    L(\pi(P);\Dcal)-V^{\pi(P)}_{P^*}\right]. 
\end{align}
In the online setting, the final Bayesian regret bound is essentially calculated by the above equation since we can control $L(\pi(P);\Dcal)-V^{\pi(P)}_{P^*}$ based on the frequentist regret bound results \citep{RussoDaniel2014LtOv}. In the offline setting, the form \eqref{eq:optimisim} is not desirable. The difference between \eqref{eq:optimisim} and \eqref{eq:pessimism} is that the policy we evaluate is $\pi(P^{*})$ in \eqref{eq:pessimism}, but it is $\pi(P)$ in \eqref{eq:optimisim}. %
 Since $\pi(P^{*})$ in \eqref{eq:pessimism} is a fixed quantity, we can use partial coverage to bound the r.h.s in \eqref{eq:pessimism}. 
\end{remark}

Finally, we remark that \pref{alg:main_alg_bonus2} would be not practical since this is a single-shot algorithm. More concretely, it is not robust to the error in a single model from $\beta(\cdot\mid \Dcal)$, i.e., it might output the poor policy $\pi^P$ if the sampled model $P$ is poor. This is easily fixed by considering $1/T\sum_{t=1}^{T}\pi(P_t)$, where $\{P_t\}_{t=1}^T$ is an i.i.d set of samples from $\beta(\cdot \mid \Dcal)$. However, this algorithm is still not practical since we need some oracle procedure for policy optimization to output $\pi^P$ given $P$. In the previous section, we instead develop the more practical algorithm PO-PS. We show PO-PS has the same guarantee as \pref{thm:naive} under the partial coverage. 
\wen{this does sound like a criticism  for the Bayesian regret itself --- the PS-PO algorithm will have this Bayesian regret as well...my suggestion is that let's just use this navie algorithm as a warm start for our analysis (do not put too much emphasize on it), but mainly focus on the PS-PO algorithm and its analysis. At the end, we can try to point out the issues of Bayesian regret..}
 
\subsection{PO-PS }





We analyze PO-PS in detail. As in the previous section, we first introduce $L(\pi;\Dcal):\Pi \to[0,H]$. Then, we assume the following.  
\begin{assum}\label{assum:lcb}
Given a model $P^{\star}$ on the support $\{P^{\star}:\beta(P^{\star})>0\}$, let $\Dcal$ be the dataset generated following $P^{\star}$. We have a function $L(\pi;\Dcal):\Pi\to [0,H]$ s.t. with probability $1-\delta$, $L(\pi;\Dcal)\leq V^{\pi}_{P^{\star}}\forall \pi\in \Pi$. 
\end{assum}

We have the following lemma for bounding per-iteration regret:
\begin{lemma}
[Per-iteration regret]
Suppose Assumption \pref{assum:lcb}. For any iteration $t$, we have 
\begin{align*}
\mathbb{E}\left[ V^{\pi(P^\star)}_{P^\star} - V^{\pi^t}_{P^\star} \right] \leq \mathbb{E}\left[ V^{\pi(P^\star)}_{P^\star} - L( \pi(P^\star);\Dcal) \right] + \mathbb{E}\left[ V^{\pi(P^{\star})}_{P^\star} - V^{\pi^t}_{P^\star}  \right]+2\delta H. 
\end{align*}\label{lem:regret}
\end{lemma}
The proof is similarly done as the proof of \pref{thm:naive}. We use a key relation $\EE[L(\pi(P^\star);\Dcal ) \mid \Dcal]=\EE[L(\pi(P_t);\Dcal ) \mid \Dcal]$. The first term is upper-bounded under the partial coverage following the argument after \pref{thm:naive}. The third term is negligible by taking sufficiently small $\delta$. Thus, we analyze the second term of r.h.s in detail. The second term corresponds to the regret term for soft policy update. This is upper-bounded by the performance gap between the policy $\pi_t$ and $\pi(P^{\star})$ under the model $P^\star$ as follows. 



\begin{lemma}\label{lem:npg}
Consider a fixed iteration $t$. Suppose $\eta<1/2H$. We have:
\begin{align*}
\mathbb{E}\left[ V^{\pi(P^{\star})}_{P^\star} - V^{\pi^t}_{P^\star}  \right] \leq \mathbb{E}\left[ \eta H^2 + \frac{H}{\eta} \mathbb{E}_{s\sim d^{\pi(P^\star)}_{P^\star},a\sim \pi(P^{\star})(s) } \left(\KL\left(\pi(P^{\star})(\cdot | s), \pi^{t+1}(\cdot | s)\right) -\KL\left( \pi(P^{\star})(\cdot|s) , \pi^{t}(\cdot | s)\right)  \right)  \right]
\end{align*}
\end{lemma}

By combining the above two lemmas, we conclude the following general theorem. 
\begin{theorem}
Suppose we have a set of functions $\Lcal_{\Dcal} \subset  \Scal\times \Pi \mapsto \mathbb{R}$ which satisfies Assumption \pref{assum:lcb}. Then, 
\begin{align*}
\mathbb{E}\left[  V^{\pi(P^\star)}_{P^\star} - \max_{t\in[T]} V^{\pi^t}_{P^\star}     \right] \leq \underbrace{\min_{L\in \Lcal_{\Dcal}}  \mathbb{E} \left[  V^{\pi(P^\star)}_{P^\star} - L( \pi(P^\star);\Dcal)\right]}_{\text{S(1)}}+\underbrace{ 4H^2 \sqrt{ \frac{ \log(|\Acal|)}{T}}}_{\text{S(2)}}+2\delta H. 
\end{align*}
\end{theorem}

By taking sufficiently large $T$, the second term (S2) is also negligible. Thus, the first term (S1) dominates the error. In the next section, we analyze the term (S1) in detail under the partial coverage. 





\subsection{Examples: Tabular MDPs, KNRs, GPs, discrete models, and low-rank models }\label{sec:example}

We can take any $L(\pi;\Dcal)$ satisfies Assumption \pref{assum:lcb}. Here, we take $\min_{M\in \Mcal_{\Dcal}}V^{\pi}_{M}$ for discrete models, KNRs, GPs in \pref{alg:main_version} and $V^{\pi}_{\hat P,r-b}$ in \citep{ChangJonathanD2021MCSi} for tabular MDPs. We can ensure the Bayesian sub-optimatliy gap bounds for these models under (Bayesian) partial coverage. 
Here, we use Bayesian concentrability coefficients \eqref{eq:Bayesian}. 



\begin{corollary}[Discrete models] \label{cor:discrete_bayes}
Suppose the partial coverage $C^{\text{Bayes}}_{\pi^{\star}}<\infty$. 
 \begin{align*}
     \mathbb{E}\left[  V^{\pi(P^\star)}_{P^\star} - \max_{t\in[T]} V^{\pi^t}_{P^\star}     \right]\leq c\prns{H^2   C^{\text{Bayes}}_{\pi^{\star}}\sqrt{\frac{\log(3|\Mcal|n)}{n} }+  H^2 \sqrt{ \frac{ \log(|\Acal|)}{T}}+\frac{H}{n}}. 
 \end{align*}
\end{corollary}


\begin{corollary}[Tabular MDPs] \label{cor:linear_bayes}
Suppose the partial coverage $C^{\text{Bayes}}_{\pi^{\star}}<\infty$. 
 \begin{align*}
    \mathbb{E}\left[  V^{\pi(P^\star)}_{P^\star} - \max_{t\in[T]} V^{\pi^t}_{P^\star}     \right] \leq  c_1 H^2\log(|\Scal||\Acal|c_2n) \prns{ \sqrt{\frac{ C^{\text{Bayes}}_{\pi^{{\star}}} |\Scal|^2|\Acal|}{n}}+\frac{ C^{\text{Bayes}}_{\pi^{{\star}}}|\Scal||\Acal|}{n}}+  4H^2 \sqrt{ \frac{ \log(|\Acal|)}{T}}+\frac{2H}{n}, 
 \end{align*}
where $c_1$ and $c_2$ are some universal constants. 
\end{corollary}

\begin{corollary}[KNRs] \label{cor:linear_bayes}
 Assume $\|\phi(s,a)\|_2\leq 1,\forall(s,a)\in \Scal\times \Acal$. Suppose the partial coverage $\bar C^{\text{Bayes}}_{\pi^{\star}}<\infty$ By letting $\|W^\star\|^2_2=O(1),\zeta^2=O(1)$,  we have 
\begin{align*}
     \mathbb{E}\left[  V^{\pi(P^\star)}_{P^\star} - \max_{t\in[T]} V^{\pi^t}_{P^\star}     \right] \leq c_1 H^2 \min(d^{1/2},  \bar R)\sqrt{ \bar R }   \sqrt{\frac{d_{\Scal}\bar C^{\Bayes}_{\pi^{{\star}}}\log (1+n) }{n}}+  4H^2 \sqrt{ \frac{ \log(|\Acal|)}{T}}+\frac{2H}{n}, 
\end{align*}
where $c_1$ and $c_2$ are some universal constants and $\bar R=  \mathrm{rank}[\Sigma_{\rho}]\{\mathrm{rank}[\Sigma_{\rho}] +\log(c_2n)\}$. 
\end{corollary}



\begin{corollary}[GPs] \label{cor:gps_bayes}
Suppose the partial coverage $\bar C^{\text{Bayes}}_{\pi^{\star}}<\infty$. By letting $\zeta^2=O(1)$,  we have 
\begin{align*}
   \mathbb{E}\left[  V^{\pi(P^\star)}_{P^\star} - \max_{t\in[T]} V^{\pi^t}_{P^\star}     \right] \leq    c_1 H^2\{d^{\star}+\log(c_2n)\}d^{\star}\sqrt{\frac{d_{\Scal}\bar C^{\Bayes}_{\pi^{{\star}}}\log^3(c_2d_{\Scal}n^2)\log (1+n) }{n}}+  4H^2 \sqrt{ \frac{ \log(|\Acal|)}{T}}+\frac{2H}{n}, 
\end{align*}
where $c_1$ and $c_2$ are some universal constants. 
\end{corollary}

\wen{add a corollary for low-rank MDP as well..}






==> analysis_flambe.tex <==
\subsection{Beyond Linear: Representation learning in low-rank MDP}


Here we attempt to do the general setting where $\phi^\star$ is not necessarily a simplex feature. 

\wen{new here: we will use MLE to construct a version space}. 

Denote $\widehat{P}_{mle}$ as the MLE solution:
\begin{align*}
\widehat{P}_{mle} := \argmin_{(\mu,\phi) \in \Mcal} \mathbb{E}_{\Dcal} -\ln \mu(s')^{\top} \phi(s,a).
\end{align*}
The MLE guarantee gives us the following generalization bound (see Flambe)
\begin{align*}
\mathbb{E}_{s,a\sim \rho,s'\sim P^\star(s,a)} \left\|  \widehat{P}_{mle}(s,a) - P^\star(s,a)     \right\|^2_1 \leq \frac{ \ln(|\Mcal| / \delta) }{ N}.
\end{align*}

Hence, we construct the version space using $\Dcal$ and $\widehat{P}_{mle}$ as follows:
\begin{align*}
\Mcal_{\Dcal} := \left\{ P \in \Mcal: \mathbb{E}_{\Dcal} \| P(s,a) - \widehat{P}_{mle}(s,a)  \|^2_{1} \leq \xi \right\}.
\end{align*}
Setting $\xi \approx 2 \frac{ \ln(|\Mcal| / \delta) }{ N}$ should be enough to guarantee that $P^\star \in \Mcal_{\Dcal}$. Thus pessimism is still guaranteed in the sense that given any policy $\pi$, $\min_{P\in\Mcal_{\Dcal}} V^{\pi}_{P}$ is a pessimistic estimate of $V^{\pi}_{P^\star}$. 


Also for any $P \in \Mcal_{\Dcal}$, we must have via triangle inequality:
\begin{align*}
\EE_{\Dcal} \| P(s,a) - P^\star(s,a) \|_1^2 \leq 2 \EE_{\Dcal} \| P(s,a) - \widehat{P}_{mle}(s,a) \|_1^2 + 2\EE_{\Dcal} \| P^\star(s,a) - \widehat{P}_{mle}(s,a) \|_1^2 \leq 4 \xi.
\end{align*} 
Thus, via concentration inequality, we must have:
\begin{align*}
\EE_{s,a\sim \rho} \| P(s,a) - P^\star(s,a)  \|_1^2 \leq c \xi, 
\end{align*} where $c$ is some constant. 

Denote $\widehat{P}$ as the $\argmin_{P\in\Mcal_{\Dcal}} V^{\pi^{\star}_{P^\star}}_{P}$. We have:
\begin{align*}
\mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 & = \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}} \mathbb{E}_{s\sim P^\star(\tilde{s},\tilde{a}), a\sim \pi^\star_{P^\star}(.|s) }\| \widehat{P}(s,a) - P^\star(s,a) \|_1 \\
& \leq A \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}} \mathbb{E}_{s\sim P^\star(\tilde{s},\tilde{a}), a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|_1 \\
& =  A{ \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left( \phi^\star(\tilde{s},\tilde{a}) \right)^{\top} \int_{s} \mu^\star(s) \EE_{a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|^2_1}
\end{align*}

Denote $\Sigma_{\rho} = \mathbb{E}_{s,a\sim \rho} \phi^\star(s,a) (\phi^\star(s,a))^{\top}$, and $\Sigma = \Sigma_{\rho} + \lambda I$. We apply CS inequality in the above inequality, 
\begin{align*}
&{ \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left( \phi^\star(\tilde{s},\tilde{a}) \right)^{\top} \int_{s} \mu^\star(s) \EE_{a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|^2_1} \\
& \leq { \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left\| \phi^\star(\tilde{s},\tilde{a})\right\|_{\Sigma^{-1}}  \underbrace{\left\|  \int_{s} \mu^\star(s) \EE_{a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|^2_1  \right\|_{\Sigma}    }_{\text{term a}}     }
\end{align*}

Let us deal with term a first. 
\begin{align*}
&\left\|  \int_{s} \mu^\star(s) \EE_{a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|^2_1  \right\|^2_{\Sigma}  \\
& \leq \mathbb{E}_{\tilde{s},\tilde{a}\sim \rho} \left( \int_{s} \mu^\star(s)^{\top} \phi^\star(\tilde{s},\tilde{a}) \EE_{a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|^2_1\right)^2 + \lambda d \\
& \leq  \mathbb{E}_{\tilde{s},\tilde{a}\sim \rho} \mathbb{E}_{s\sim P^\star(\tilde{s},\tilde{a}),a\sim U(\Acal)}   \| \widehat{P}(s,a) - P^\star(s,a)  \|_1^4 + \lambda d \\
& \leq  4 \mathbb{E}_{\tilde{s},\tilde{a}\sim \rho} \mathbb{E}_{s\sim P^\star(\tilde{s},\tilde{a}),a\sim U(\Acal)}   \| \widehat{P}(s,a) - P^\star(s,a)  \|_1^2 + \lambda d \\
& \leq \frac{ \ln(|\Mcal| / \delta )}{N} + \lambda d.
\end{align*}

Plug in term a back, we get:
\begin{align*}
&{ \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left( \phi^\star(\tilde{s},\tilde{a}) \right)^{\top} \int_{s} \mu^\star(s) \EE_{a\sim U(\Acal)}\| \widehat{P}(s,a) - P^\star(s,a) \|^2_1} \\ 
& \leq { \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left\| \phi^\star(\tilde{s},\tilde{a})\right\|_{\Sigma^{-1}}   } \left(  \frac{ \ln(|\Mcal| / \delta )}{N} + \lambda d  \right)^{1/2}
\end{align*}

Now we can use relative condition number to deal with the first term above.
\begin{align*}
&\mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left\| \phi^\star(\tilde{s},\tilde{a})\right\|_{\Sigma^{-1}}  \leq \sqrt{ \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \left\| \phi^\star(\tilde{s},\tilde{a})\right\|^2_{\Sigma^{-1}} } \\
& =\sqrt{  \tr\left( \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \phi^\star(\tilde{s},\tilde{a}) \phi^\star(\tilde{s},\tilde{a})^{\top} \Sigma^{-1}   \right) } \leq \sqrt{ C \tr\left( \Sigma_{\rho} \Sigma^{-1}  \right)} \leq \sqrt{Cd}.
\end{align*}

Combine all the above results together, we get:
\begin{align*}
\mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \left\| \widehat{P}(s,a) - P^\star(s,a) \right\|_1  \leq A  \left( \sqrt{Cd } \cdot  \left(  \frac{ \ln(|\Mcal| / \delta )}{N} + \lambda d  \right)^{1/2}  \right)
\end{align*}
We can set $\lambda \eqsim 1/ (Nd)$, which gives the following bound:
\begin{align*}
\mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \left\| \widehat{P}(s,a) - P^\star(s,a) \right\|_1 \leq A \sqrt{  \frac{ C d  \ln(|\Mcal| / \delta) }{ N}    }.
\end{align*}





==> analysis_flambe_simplex.tex <==
\subsection{Beyond Linear: Representation learning in low-rank MDP}


In feature selection problem, we consider MDPs with low-rank structure. We explain the setting in the frequentist setting first and then state our result in Bayesian setting.  

\begin{definition}[Latent state representation (i.e., MDP with low NNR)]
Consider a fixed model $P^\star$ and the dataset $\Dcal$ generated based on $P^\star$. The transition operator has a latent representation if there exists a latent space $\Zcal$, and  two functions $\mu: \Zcal\mapsto \Delta(\Scal)$, and $\phi:\Scal\times\Acal\mapsto \Delta(\Zcal)$, such that for any $(s,a)$, $P^\star(\cdot | s,a) = \sum_{z\in\Zcal} \mu(\cdot | z) \phi(z | s,a)$.  Let $d$ denote the cardinality of the smallest $\Zcal$ that admits the above latent representation.  Note that $d$ is essentially the non-negative matrix rank of the transition operator $P^\star\in\mathbb{R}^{|\Scal|\times|\Scal||\Acal|}$.
\end{definition}

Given a dataset $\Dcal$ sampled from $P^\star$, we explain how we could maintain a version space over $\Mcal$.

We define $\Fcal = \Scal\times\Acal\times\Scal \mapsto [0,1]$ as a set of discriminators. We define $\ell$ as a discrepancy function:
\begin{align*}
\ell(s,a,s', P, \nu) := \mathbb{E}_{s''\sim P(s,a)} \nu(s,a,s'') - \nu(s,a,s').
\end{align*}
Denote $\pi_{b}$ as the behavior policy that induces the offline distribution $\rho(s,a)$ (i.e., $\rho = d^{\pi_b}_{P^\star}$). We construct the discriminator functions as follows.  For any two pairs of models $P$ and $P'$ in $\Mcal$, we define $\nu_{P,P'}$ as the witness function:
\begin{align*}
\nu_{P, P'} = \argmax_{\nu\in \Fcal} \mathbb{E}_{s,a\sim d^{\pi_b}_{P'}} \mathbb{E}_{s''\sim P(s,a)} \nu(s,a,s') - \mathbb{E}_{s,a\sim d^{\pi_b}_{P'}} \mathbb{E}_{s'\sim P'(s,a)} \nu(s,a,s').  
\end{align*} We enumerate all different pairs of $P, P'$ ($P \neq P'$), and refine $\Fcal$ as:
\begin{align*}
\Fcal = \{ \nu_{P, P'} : P \in \Mcal, P' \in \Mcal, P \neq P' \}.
\end{align*}

Why we construct such $\Fcal$? First such $\Fcal$ has bounded complexity now. Secondly, it is still rich enough to model the total variation distance, i.e., 
\begin{align*}
& \max_{ \nu \in \Fcal} \left[ \mathbb{E}_{s,a\sim \rho} \mathbb{E}_{s'\sim P(s,a)}  \nu(s,a,s') - \mathbb{E}_{s,a\sim \rho} \mathbb{E}_{s'\sim P^\star(s,a)} \nu(s,a,s')   \right] \\
& =  \mathbb{E}_{s,a\sim \rho} \mathbb{E}_{s'\sim P(s,a)}  \nu_{P,P^\star}(s,a,s') - \mathbb{E}_{s,a\sim \rho} \mathbb{E}_{s'\sim P^\star(s,a)} \nu_{P,P^\star}(s,a,s')  \\
& = \left\| \rho P - \rho P^\star    \right\|_1 = \mathbb{E}_{s,a\sim \rho} \| P(s,a) - P^\star(s,a)  \|_1.
\end{align*}


With this setup, we consider the following version space:
\begin{align*}
\Mcal_{\Dcal} = \left\{  P \in \Mcal:   \max_{\nu\in\Fcal} \mathbb{E}_{\Dcal} \ell(s,a,s', P, \nu) \leq \xi  \right\},
\end{align*} where $\xi \in \mathbb{R}^d$ is a statistical error that is related to the number of samples in $\Dcal$, which we will specify later. 

Now we show that with $\xi$ being set properly, we can show that $P^\star \in \Mcal_{\Dcal}$.
\begin{lemma}[Feasibility] \label{lem:feasible}Set $\xi =2 \ell_{\max} \sqrt{\frac{ \ln(|\Mcal|^3/ \delta)  }{N}}$, with probability at least $1-\delta$, we have $P^\star \in \Mcal_{\Dcal}$, where the randomness is with respect to the randomness in $\Dcal$.
\end{lemma}
\begin{proof}
Via Hoeffding's inequality, and a union bound over $\Mcal$ and $\Fcal$,  we have:
\begin{align*}
\left\lvert \mathbb{E}_{s,a\sim \rho, s'\sim P^\star(s,a)} \ell(s,a,s', P, \nu) - \mathbb{E}_{\Dcal} \ell(s,a,s', P, \nu) \right\rvert \leq 2\ell_{\max} \sqrt{\frac{ \ln( |\Mcal| |\Fcal|/\delta) }{N}}, 
\end{align*}with probability $1-\delta$.

Since for any $\nu$, we have $\mathbb{E}\ell(s,a,s', P^\star, \nu) = 0$, we have:
\begin{align*}
\max_{\nu} \mathbb{E}_{\Dcal} \ell(s,a,s', P^\star, \nu) \leq2\ell_{\max} \sqrt{\frac{ \ln( |\Mcal| |\Fcal|/\delta) }{N}}.
\end{align*}
Now use the fact that $|\Fcal| = |\Mcal|^2$, we conclude the proof.
\end{proof}

Condition on the event in \pref{lem:feasible} being true, we immediately get LCB for any policy $\pi$. For any $\pi$, we set its LCB as $ \min_{P\in\Mcal_{\Dcal}} V^{\pi}_{P}$. Since $P^\star \in \Mcal_{\Dcal}$, we have $\min_{P\in\Mcal} V^{\pi}_{P} \leq V^{\pi}_{P^\star}$. Note that this holds for all $\pi$.




To bound the regret, we introduce a definition of partial coverage for the latent representation model. Specifically, we will define concentrability coefficient in the latent state space $\Zcal$, and the concentrability coefficient only concerns $\pi^\star_{P^\star}$ and $\rho$, i.e., we simply require that the latent state distribution induced by $\rho$ covers the latent state distribution induced by the optimal policy $\pi^\star_{P^\star}$ --- thus partial coverage. 

\begin{assum}[Partial concentrability coefficient in latent state space] Denote $\rho(z)$ as the latent distribution over $\Zcal$ induced by $\rho$, i.e., $\rho(z) = \mathbb{E}_{s,a\sim \rho} \phi^\star(z | s,a)$, and similarly $d^{\pi^\star_{P^\star}}_{P^\star}(z) := \mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \phi^\star(z|s,a)$. We assume that following concentrability coefficient is bounded:
\begin{align*}
\max_{z\in\Zcal} \frac{ d^{\pi^\star_{P^\star}}_{P^\star}(z) }{ \rho(z)} \leq C_{P^\star} < \infty.
\end{align*}\label{assum:partial_coverage}
\end{assum}

 Note that since $\Scal$ could be extremely large, the above bounded latent state space concentrability coefficient is a much weaker assumption than the bounded concentrability coefficient in the original state space $\Scal$; also note that $C_{P^\star}$ only concerns $d^{\pi^\star_{P^\star}}_{P^\star}$, i.e., we only require $\rho$ to coverage the comparator $\pi^\star_{P^\star}$.



Now we use the property of low rankness in $P^\star$.  For simplicity, we assume $\rho$ is the stationary state-action distribution of the behavior policy $\pi_b$.  Denote $\widehat{P} = \argmin_{P\in\Mcal_{\Dcal}} V^{\pi}_{P} $.  Since $\widehat{P} \in \Mcal_{\Dcal}$, we must have:
\begin{align*}
&\max_{\nu\in\Fcal} \mathbb{E}_{s,a\sim \rho,s'\sim P^\star(s,a)} \ell(s,a,s', \widehat{P}, \nu) \\
&\leq  \max_{\nu\in\Fcal} \mathbb{E}_{s,a\sim \rho,s'\sim P^\star(s,a)} \ell(s,a,s', \widehat{P}, \nu) + 2\ell_{\max} \sqrt{\frac{\ln(|\Mcal| / \delta)}{N}} \leq  4 \ell_{\max} \sqrt{\frac{\ln(|\Mcal| / \delta)}{N}}  = 4 \xi.
\end{align*}
Recall the property of the refined $\Fcal$, we know that $\max_{\nu\in\Fcal} \mathbb{E}_{s,a\sim \rho,s'\sim P^\star(s,a)} \ell(s,a,s', \widehat{P}, \nu) = \mathbb{E}_{s,a\sim \rho} \| \widehat{P}(s,a) - P^\star(s,a)  \|_1  $. Thus, we have:
\begin{align*}
\mathbb{E}_{s,a\sim \rho} \| \widehat{P}(s,a) - P^\star(s,a)  \|_1  \leq  4\xi.
\end{align*}
Using the one-step back trick, we have:
\wen{for the non simplex case, maybe  we can do $\EE \sqrt{a^2} \leq \sqrt{ \EE[a^2] }$}
\begin{align*}
\mathbb{E}_{s,a\sim \rho} \| \widehat{P}(s,a) - P^\star(s,a)  \|_1&  = \mathbb{E}_{\tilde{s},\tilde{a}\sim \rho} \mathbb{E}_{s\sim P^\star(\tilde{s},\tilde{a}), a\sim \pi_b(.|s)} \left\| \widehat{P}(s,a) - P^\star(s,a)  \right\|_1 \\
& = \mathbb{E}_{\tilde{s},\tilde{a}\sim \rho}   \sum_{z\in\Zcal} \phi^\star(z | \tilde{s},\tilde{a}) \int_{s} \mu^\star(s | z)  \mathbb{E}_{a\sim \pi_b(.|s)} \left\| \widehat{P}(s,a) - P^\star(s,a)  \right\|_1 \\
& = \sum_{z\in\Zcal}  \rho(z) \int_{s} \mu^\star(s | z)  \mathbb{E}_{a\sim \pi_b(.|s)} \left\| \widehat{P}(s,a) - P^\star(s,a)  \right\|_1 \\
& \geq \left( \min_{a,s} \pi_b(a|s) /A  \right) \sum_{z\in\Zcal}  \rho(z) \int_{s} \mu^\star(s | z)  \mathbb{E}_{a\sim U(\Acal)} \left\| \widehat{P}(s,a) - P^\star(s,a)  \right\|_1
\end{align*} where the last inequality changes from $\pi_b$ to $U(\Acal)$ and it holds since $\mu^\star(s|z) \geq 0$ (due to the latent state representation definition).
Re-arrange terms, we get:
\begin{align*}
\sum_{z\in\Zcal}  \rho(z) \int_{s} \mu^\star(s | z)  \mathbb{E}_{a\sim U(\Acal)} \left\| \widehat{P}(s,a) - P^\star(s,a)  \right\|_1 \leq \frac{4 A \xi}{  \min_{a,s} \pi_b(a|s) }.
\end{align*}





Now we look at the objective function that we want to upper bound, i.e., $V^{\pi^\star_{P^\star}}_{P^\star} - V^{\pi^\star_{P^\star}}_{\widehat{P}}$. Via simulation lemma, we must have:
\begin{align*}
V^{\pi^\star_{P^\star}}_{P^\star} - V^{\pi^\star_{P^\star}}_{\widehat{P}} \leq H^2 \mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \| \widehat{P}(s,a) - P^\star(s,a) \|_1
\end{align*} We use the one-step back trick again assuming $d^{\pi^\star_{P^\star}}_{P^\star}$ is a stationary distribution \wen{we need to fix this by using the initial state distribution..or time dependent model..}:
\begin{align*}
\mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \| \widehat{P}(s,a) - P^\star(s,a) \|_1& = \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \sum_{z\in\Zcal} \phi^\star(z | s,a) \int_{s} \mu^\star(s | z) \mathbb{E}_{a\sim \pi^\star_{P^\star}(.|s)} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 \\
& \leq A \mathbb{E}_{\tilde{s},\tilde{a}\sim d_{P^\star}^{\pi^\star_{P^\star}}}  \sum_{z\in\Zcal} \phi^\star(z | s,a) \int_{s} \mu^\star(s | z) \mathbb{E}_{a\sim U(\Acal)} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 \\
& = A  \sum_{z\in \Zcal} d^{\pi^\star_{P^\star}}_{P^\star}(z)   \int_{s} \mu^\star(s | z) \mathbb{E}_{a\sim U(\Acal)} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 .
\end{align*}




Now we can link the above two results together using Assumption~\pref{assum:partial_coverage}. 
\begin{align*}
V^{\pi^\star_{P^\star}}_{P^\star} - V^{\pi^\star_{P^\star}}_{\widehat{P}}  & \leq H^2 \mathbb{E}_{s,a\sim d_{P^\star}^{\pi^\star_{P^\star}}} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 \leq H^2 A \sum_{z\in \Zcal} d^{\pi^\star_{P^\star}}_{P^\star}(z)   \int_{s} \mu^\star(s | z) \mathbb{E}_{a\sim U(\Acal)} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 \\
& = H^2 A \sum_{z\in\Zcal} \frac{ d^{\pi^\star_{P^\star}}_{P^\star}(z) }{\rho(z)} \rho(z) \int_{s} \mu^\star(s | z) \mathbb{E}_{a\sim U(\Acal)} \| \widehat{P}(s,a) - P^\star(s,a) \|_1 \\
& \leq C_{P^\star} H^2 A \mathbb{E}_{z\sim \rho} \int_{s} \mu^\star(s | z) \mathbb{E}_{a\sim U(\Acal)} \| \widehat{P}(s,a) - P^\star(s,a) \|_1  \\
& \leq \frac{ 4 C_{P^\star} H^2 A^2 \xi  }{ \min_{s,a} \pi_b(a|s)} =  \frac{ 4 C_{P^\star} H^2 A^2   }{ \min_{s,a} \pi_b(a|s)}  \cdot  \ell_{\max} \sqrt{ \frac{ \ln(|\Mcal|^3 / \delta) }{N}  }.
\end{align*}

\wen{the bound does not dependent on rank $d$ ??? weird, but i cannot see where it is wrong..}

\wen{can we get rid of the simple feature assumption? one issue is that $\mu^\star$ is not necessarily gonna be positive anymore in the general case..there are also other issues in terms of how to get the log det potential form..}




==> conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion}
\vspace{-0.2cm}
We study model-based offline RL with function approximation under partial coverage. We show that for the model-based setting, realizability in function class and partial coverage together are enough to learn a policy that is comparable to \emph{any} policies (including history-dependent policies) covered by the offline distribution. Our result demonstrates a sharp contrast to model-free offline RL approaches which often require additional structural conditions in the function class (e.g., Bellman completion) and have restrictions on the pool of candidate policies that they can compete against. 

Some readers might wonder whether CPPO is computationally efficient. The minimax optimization problem $\argmax_{\pi \in \Pi}\min_{P\in M}V^{\pi}_P$ fits into a framework of planning on robust MDPs \citep{nilim2005robust,iyengar2005robust}. By introducing a robust Bellman equation, they proposed value iteration and policy iteration algorithms, and showed that algorithms are practically tractable in the tabular setting. In the non-tabular setting, \citet{lim2019kernel,tamar2014scaling} propose the extension using function approximation. Thus, we can apply their methods to approximately solve the minimax optimization problem in a model-free fashion. We leave the formal theoretical justification when using these approximation planning algorithms as an important direction for future work. 






==> generalization_old.tex <==
\section{Generalization}\label{sec:general}

We explain how to generalize \pref{thm:version} when the hypothesis class is infinite. MLE has the following guarantee. 
Here, the localized Rademacher complextiy for a function class $\Fcal$ is defined as 
\begin{align*}
    \Rcal_n(\delta;\Fcal)\coloneqq \EE_{x,\epsilon}\bracks{ \sup_{g\in \Fcal,\EE[g^2]\leq \delta}\left|\frac{1}{n}\sum_i \epsilon_ig(x_i) \right| }
\end{align*}
where $\epsilon_i$ is a i.i.d set of Rademacher variables. In our problem, $x_i=\{s_i,a_i,s'_i\}$ and the expectation is taken w.r.t $x\sim \rho(s,a)P^{*}(s'\mid s,a)$. 

\begin{theorem}\label{thm:mle}
Let $  \Hcal=\{\sqrt{P/P^{*}}\mid P\in \Mcal\}.  $ Suppose $0<b_1\leq \|P(s'|s,a)\|_{\infty}\leq b_2$ for any $P\in \Mcal$,  $P^{*}(s'\mid s,a)\geq b_3>0$ for any $s,a,s'$. Additionally, assume $\Hcal$ is star-shaped around $1$. Let $D_n$ be any solution w.r.t $\delta$ to the following critical inequality:
\begin{align*}
    \Rcal_n(\delta;\Hcal-1)\leq \frac{\delta^2}{\sqrt{b_1/b_2}}.  
\end{align*}
Then, with probability $1-\delta$,  we have $$\EE_{(s,a)\sim \rho}[\|\hat P_{\MLE}(s'\mid s,a)-P(s'\mid s,a)\|^2_1]\leq c\{D_n+\sqrt{\log(1/\delta)/n}\}^2,$$
where $c$ is some universal constant. 
\end{theorem}

For example, when the hypothesis class is finite, we have $D_n=\sqrt{\log(|\Mcal|/\delta)/n}$. 



\begin{proof}
We use \citep[Theorem 14.20]{WainwrightMartinJ2019HS:A}.  We need to check two assumptions in \citet[Page 470]{WainwrightMartinJ2019HS:A}. 
We consider a loss function $L(x)=-\log h(x)$ on $\Hcal$. Then, this loss function is $\sqrt{b_1 b_3}$-Lipchitz since 
\begin{align*}
    |L_h(s,a,s') -L_{\tilde h}(s,a,s') |\leq \sqrt{b_1b_3}|h(s'|s,a)-h(s'|s,a)|,\forall (s,a,s'),\forall h, \tilde h\in \Hcal. 
\end{align*}
noting mean-value theorem and $h(s'|s,a)\geq \sqrt{b_1b_3} (\forall (s,a,s'))$. Besdies, this loss-function is $0.5$-strongly-convex around the true value $h^{*}=P^{*}/P^{*}=1$ in the sense that  
\begin{align*}
    &\EE\bracks{L_h(s,a,s') -L_{h^{*}}(s,a,s')-\frac{1}{h^{*}(s,a,s')}(h-h^{*})}\\
    &=\EE\bracks{\frac{1}{2}\log \frac{P^{*}(s'\mid s,a)}{P(s'\mid s,a)} }=\frac{1}{2}\EE_{(s,a)\sim \rho}[\mathrm{KL}((P^{*}(\cdot\mid s,a)\| P(\cdot\mid s,a))]\\ 
    &\geq \EE_{(s,a)\sim \rho}[\mathrm{H}^2 (P^{*}(\cdot\mid s,a)\| P(\cdot\mid s,a)) ]=0.5\EE[(h(s,a,s')-h^{*}(s,a,s'))^2]. 
\end{align*}
where $\mathrm{H}^2(a\| b)$ means Hellinger distance between $a$ and $b$. Thus, we can invoke \citep[Theorem 14.20]{WainwrightMartinJ2019HS:A}. Then, with probability $1-\delta$,  we have 
\begin{align*}
\EE_{(s,a)\sim \rho}[\mathrm{H}^2 (P^{*}(\cdot\mid s,a)\|\hat P_{\MLE}(\cdot\mid s,a)) ]\leq c\{D_n+\sqrt{\log(1/\delta)/n}\}. 
\end{align*}
This implies 
\begin{align*}
   \EE_{(s,a)\sim \rho}[\|\hat P_{\MLE}(\cdot\mid s,a)-P(\cdot\mid s,a)\|^2_1]\leq c\{D_n+\sqrt{\log(1/\delta)/n}\}^2.
\end{align*}
\end{proof}




Then, based on the notation of \pref{thm:mle}, we have the following theorem. 
\begin{theorem}\label{thm:version2}
We suppose the assumption in \pref{thm:mle}. 
Assume $P^{*}\in \Mcal$. We set $\xi=c\{D_n+\sqrt{\log(1/\delta)/n}\}$.  For any comparator policy $\pi^*$ (not necessarily the optimal one),  define the concentrability coefficient $C_{\pi^{*}} :=\max_{(s,a)\in \Scal\times \Acal}\frac{d^{\pi}_{P^{*}}(s,a) }{\rho(s,a)}.$ Suppose $C_{\pi^{*}}<\infty$. Then, with probability $1-\delta$, 
\begin{align*}
      V^{\pi^{*}}_{P^{*}}-V^{\hat \pi}_{P^{*}} \leq  3\xi H C^{\dagger}_{\pi^{*}},\quad C^{\daggeer}=\sup_{P\in \Mcal-\Mcal}\frac{\EE[\|P(\cdot\mid s,a\|_1 ] }{}
\end{align*}
\end{theorem} 
This is proved as \pref{thm:version}. 

==> pg_proof.tex <==

\section{Missing Proofs in \pref{sec:alg} } 


Here, $P^{\star}\sim \beta(\cdot),\Dcal \sim  d(\cdot \mid P^{\star})$. Then, by denoting the posterior distribution of $P^{\star}$ given $\Dcal$ as $\beta'(\cdot\mid \cdot)$, then $P_t\sim \beta(\cdot \mid \Dcal)$. %



We start with the proof of \pref{lem:regret}. 

\begin{proof}[Proof of \pref{lem:regret}]
\begin{align*}
  \EE\bracks{  V^{\pi(P^{\star})}_{P^\star}   -  V^{\pi_t}_{P^\star}}&=\EE\bracks{ V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)+  L(\pi(P^{\star});\Dcal)- V^{\pi_t}_{P^\star} } \\ 
  &=\EE\bracks{ V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)+  \EE[L(\pi(P^{\star});\Dcal)\mid \Dcal]- V^{\pi_t}_{P^\star} } \\ 
    &=\EE\bracks{ V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)+  \EE[L(\pi(P_t);\Dcal)\mid \Dcal]- V^{\pi_t}_{P^\star} } \\ 
  &= \EE\bracks{ V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)+  L(\pi(P_t);\Dcal)- V^{\pi_t}_{P^\star} }. 
\end{align*}
From the second line to the third line, we use $\mathrm{Pr}(P^{\star}\mid \Dcal)=\beta'(P^{\star}\mid \Dcal)$, $\mathrm{Pr}(P_t\mid \Dcal)=\beta'(P_t\mid \Dcal)$. 
\end{proof}

Besides, by denoting the event $\Zcal=\{ L(\pi;\Dcal)\leq V^{\pi}_{P^{\star}},\forall \pi\in \Pi\}$ from the assumption, 
\begin{align*}
   \EE\bracks{L(\pi(P_t);\Dcal)}&=  \EE[\EE\bracks{L(\pi(P_t);\Dcal)\mid \Zcal,P^{\star}}P(\Zcal|P^{\star})]+ \EE[2H(1-P(\Zcal|P^{\star}))]\\
   &\leq \EE\bracks{\EE\bracks{V_{P^{\star}}^{\pi(P_t)} \mid \Zcal,P^{\star}} }+ 2H\delta \\
   &\leq \EE\bracks{\EE\bracks{V_{P^{\star}}^{\pi(P^{\star})} \mid \Zcal,P^{\star}} }+2H\delta\\
   &= \EE\bracks{V_{P^{\star}}^{\pi(P^{\star})} \EE\bracks{1 \mid \Zcal,P^{\star}} }+2H\delta=\EE{\bracks{V_{P^{\star}}^{\pi(P^{\star})}} }+2H\delta. 
\end{align*}
Thus, 
\begin{align*}
      \EE\bracks{  V^{\pi(P^{\star})}_{P^\star}   -  V^{\pi_t}_{P^\star}}& \leq \EE\bracks{ V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)+V^{\pi(P^{\star})}_{P^\star}- V_{P^{\star}}^{\pi_t} }+2H\delta. 
\end{align*}


Next, we prove  \pref{lem:npg}. 

\begin{proof}[Proof of \pref{lem:npg}]

\begin{align*}
\EE\bracks{V_{P^{\star}}^{\pi(P^{\star})} - V^{\pi_t}_{P^\star} }=H\EE_{(s,a) \sim d_{P^{\star}}^{\pi(P^{\star})} }[A^{\pi_t}_{P^{\star}}(s,a)] \tag{Performance difference lemma}. 
\end{align*}

Here, we have 
\begin{align*}
    &\EE_{(s) \sim d_{P^{\star}}^{\pi(P^{\star})} }\bracks{\frac{\KL( \pi(P^{\star})(\cdot \mid s),\pi_{t+1}(\cdot \mid s))-\KL(\pi(P^{\star})(\cdot \mid s),\pi_t(\cdot \mid s))}{\eta}}\\
    &= \EE_{(s) \sim d_{P^{\star}}^{\pi(P^{\star})},a\sim \pi(P^{\star})(s) }\bracks{\ln\frac{\pi^{t+1}(a\mid s)}{\pi_t(a\mid s)} }\\ 
    &=\EE_{(s) \sim d_{P^{\star}}^{\pi(P^{\star})},a\sim \pi(P^{\star})(s) }\bracks{A^{\pi_t}_{P_t}(s,a)-\frac{1}{\eta}\ln\EE_{a\sim \pi^{t}}[\exp(\eta  A^{\pi_t}_{P_t}(s,a)] } \\ 
    &\geq \EE_{(s) \sim d_{P^{\star}}^{\pi(P^{\star})},a\sim \pi(P^{\star})(s) }\bracks{A^{\pi_t}_{P_t}(s,a)}-\eta (2H)^2 . 
\end{align*}
From the second line to third line, we use the following 
\begin{align*}
    \ln\EE_{a\sim \pi^{t}(s)}[\exp(\eta  A^{\pi_t}_{P_t}(s,a)]& \leq  \ln\braces{\EE_{a\sim \pi^{t}(s)}[1+\eta  A^{\pi_t}_{P_t}(s,a)+\{\eta  A^{\pi_t}_{P_t}(s,a)\}^2] } \tag{$\eta\leq 1/(2H),\exp(x)\leq 1+x+x^2 (x\leq 1)$}\\
    & \leq \ln\braces{\EE_{a\sim \pi^{t}(s)}[1+\eta^2 (2H)^2 ] } \tag{$\log(1+x)\leq x$}\\
    &\leq \eta^2(2H)^2 . 
\end{align*}
   
Then, 
\begin{align*}
    \EE\bracks{V_{P^{\star}}^{\pi(P^{\star})} - V^{\pi_t}_{P^\star} }   &=H\EE[\EE_{(s,a) \sim d_{P^{\star}}^{\pi(P^{\star})} }[\EE[A^{\pi_t}_{P_{t}}(s,a) ]]\\
      &\leq H\EE\bracks{\EE_{(s) \sim d_{P^{\star}}^{\pi(P^{\star})} }\bracks{\eta (2H)^2 +\frac{\KL( \pi(P^{\star})(\cdot \mid s),\pi_{t+1}(\cdot \mid s))-\KL(\pi(P^{\star})(\cdot \mid s),\pi_t(\cdot \mid s))}{\eta}} }. 
\end{align*}
\end{proof} 


\begin{proof}[Proof of \pref{thm:bayesian_pspo}]
Finally, 
\begin{align*}
     & \min_{t\leq T}\EE\bracks{  V^{\pi(P^{\star})}_{P^\star}   -  V^{\pi_t}_{P^\star}}\\
     &\leq \braces{\EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ] }+\frac{1}{T}\sum_{t=1}^T     \EE\bracks{V_{P^{\star}}^{\pi(P^{\star})} - V^{\pi_t}_{P^\star} }+2H\delta\\
     &\leq \braces{\EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ] }\\
     &+H\braces{\eta (2H)^2+\frac{1}{T}\EE\bracks{\EE_{(s) \sim d_{P^{\star}}^{\pi(P^{\star})} }\bracks{\frac{\KL( \pi(P^{\star}(\cdot \mid s)),\pi_{T+1}(\cdot \mid s))-\KL(\pi(P^{\star})(\cdot \mid s),\pi_1(\cdot \mid s))}{\eta}}}}+2H\delta  \\
     &\leq \braces{\EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ] }+H\braces{\eta (2H)^2+\frac{\ln |\Acal|}{\eta T} }+2H\delta\\
     & \leq \braces{\EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ] }+4H^2\sqrt{\frac{\ln |\Acal|}{T}}+2H\delta. 
\end{align*}
Thus, 
\begin{align*}
 \min_{t\leq T}\EE\bracks{  V^{\pi(P^{\star})}_{P^\star}   -  V^{\pi_t}_{P^\star}} \leq \braces{\min_{L\in \Lcal_{\Dcal}}\EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ] }+4H^2\sqrt{\frac{\ln |\Acal|}{T}}+2H\delta. 
\end{align*}


\end{proof}


\begin{proof}[Proof of Corollary \pref{cor:discrete_bayes}]
We take $L(\pi;\Dcal)$ as $\max(\min(\min_{M\in \Mcal_{\Dcal}}V^{\pi}_{M},H),0)$ in \pref{thm:version}. Then, from the first step in the proof of \pref{thm:version}, conditional on $P^{\star}$, with probability $1-\delta$, $L(\pi;\Dcal)$ satisfies 
\begin{align*}
    L(\pi;\Dcal)\leq V^{\pi}_{P^{\star}},\forall \pi \in \Pi.  
\end{align*}
and 
\begin{align*}
    \EE_{(s,a)\sim \rho}[\|P'(s,a) - P^\star(s,a)  \|^2_1 ]\lesssim \xi. 
\end{align*}
where $P'=\argmin_{M\in \Mcal_{\Dcal}}V^{\pi(P^{\star})}_{M}$. We denote the above event as $\Zcal$. We have $\mathrm{P}(\Zcal\mid P^{\star})\geq 1-\delta$. 
In addition, from the third step in the proof of \pref{thm:version},  

\begin{align*}
   & \EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ]\leq  \tag{The third step in the proof of \pref{thm:version}} \EE[V^{\pi(P^{\star})}_{P^{\star}}-V^{\pi(P^{\star})}_{P'}] \\
       & \leq H^2\EE_{P^{\star}\sim \beta}[\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|_1 ]] \tag{Simulation lemma, \pref{lem:simulation}}\\
        &\leq H^2\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|_1 ]\mid \Zcal,P^{\star}}P(\Zcal\mid P^{\star})}+\EE_{P^{\star}\sim \beta}[2H(1-P(\Zcal\mid P^{\star}) )]\\
       &\leq H^2\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|_1 ]\mid \Zcal,P^{\star}}}+2H\delta \\
         &\leq H^2\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\sqrt{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|^2_1 ]}\mid \Zcal,P^{\star}}}+2H\delta \\
        &\leq H^2\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\sqrt{C^{\dagger}_{\pi(P^{\star}),P^{\star}}\EE_{(s,a)\sim \rho}[\|P'(s,a) - P^\star(s,a)  \|^2_1 ]}\mid \Zcal,P^{\star}}}+2H\delta \\
 &\leq H^2\sqrt{\xi}\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\sqrt{C^{\dagger}_{\pi(P^{\star}),P^{\star}}}\mid \Zcal,P^{\star}}}+2H\delta \\
  &\leq H^2\sqrt{\xi}\EE_{P^{\star}\sim \beta}\bracks{\sqrt{C^{\dagger}_{\pi(P^{\star}),P^{\star}}}\EE\bracks{1\mid \Zcal,P^{\star}}}+2H\delta\\
  &= H^2\sqrt{\xi}\sqrt{\EE_{P^{\star}\sim \beta}\bracks{C^{\dagger}_{\pi(P^{\star}),P^{\star}}}}+2H\delta. 
\end{align*}
By taking $\delta=1/n$, the statement is concluded. 
\end{proof}

\begin{proof}[Proof of Corollary  \ref{cor:tablar_bayes} ]
The proof is done as in the proof of Corollary \pref{cor:discrete_bayes}. We omit the proof. 
\end{proof}

\begin{proof}[Proof of Corollary  \ref{cor:linear_mixture_bayes} ]
The proof is done as in the proof of Corollary \pref{cor:discrete_bayes}. We omit the proof. 
\end{proof}

\begin{proof}[Proof of Corollary \ref{cor:linear_bayes}]
We take  $L(\pi;\Dcal)$ as $\max(\min(\min_{W\in \Wcal_{\Dcal}}V^{\pi}_{P(W)},H),0)$ in \pref{thm:version}. Then, from the first and second step in the proof of Corollary \pref{cor:knrs}, conditioning on $P^{\star}$, with probability $1-\delta$, $L(\pi;\Dcal)$ satisfies 
\begin{align*}
      L(\pi;\Dcal)\leq V^{\pi}_{P^{\star}},\forall \pi \in \Pi. 
\end{align*}
and  $$ \left\| \left(W' - W^\star\right) \left(\Sigma_{n}\right)^{1/2}  \right\|_2\leq \xi, $$
where $W'=\argmin_{W\in \Mcal_{\Dcal}}V^{\pi(P^{\star})}_{P(W)}$. Besides, from \citet[Theoreem 20]{ChangJonathanD2021MCSi}, with probability $1-\delta$,  we have
\begin{align*} 
  \xi \leq c_1\sqrt{1+d_{\Scal}\min(\mathrm{rank}(\Sigma_{\rho})\{\mathrm{rank}(\Sigma_{\rho})+\ln(c_2/\delta)\},d)\ln (1+n) }.
\end{align*}
In addition, from \citet[Theorem 21]{ChangJonathanD2021MCSi}, with probability $1-\delta$, we also have 
\begin{align*}
    \EE_{(s,a)\sim \rho}[\|\phi(s,a)\|_{\Sigma^{-1}_{n}}]&\leq c_1\sqrt{\frac{\mathrm{rank}[\Sigma_{\rho}]\{\mathrm{rank}[\Sigma_{\rho}] +\ln(c_2/\delta)\}}{n}}. 
\end{align*}
We denote the above event as $\Zcal$. Then, we have $P(\Zcal \mid P^{\star})\geq 1-\delta$. 


From the third step in the proof of Corollary \ref{cor:knrs},
\begin{align*}
      &\EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ]\leq \EE[V^{\pi(P^{\star})}_{P^{\star}}-V^{\pi(P^{\star})}_{P(W')}]  \\ 
      &\leq \frac{H^2}{\zeta} \EE_{P^{\star}\sim \beta}\bracks{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|(W' - W^\star) \phi(s,a)  \|_2]} \tag{Simulation lemma}\\ 
       &\leq  \frac{H^2}{\zeta} \EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|(W'  - W^\star) \phi(s,a)  \|_2] \mid P^{\star},\Zcal}}+2H\delta \\ 
         &\leq  \frac{H^2}{\zeta} \EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\xi \EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|\phi(s,a)\|_{\Sigma^{-1}_n}] \mid P^{\star},\Zcal}}+2H\delta \\  
           &\leq  \frac{H^2}{\zeta} \EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\xi \sqrt{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|\phi(s,a)\|^2_{\Sigma^{-1}_n}]} \mid P^{\star},\Zcal}}+2H\delta.
\end{align*}           
Then, by letting $ \bar R=  \mathrm{rank}[\Sigma_{\rho}]\{\mathrm{rank}[\Sigma_{\rho}] +\ln(c_2/\delta)\}$, 
\begin{align*}
             \EE[ V^{\pi(P^{\star})}_{P(W')}-V^{\pi(P^{\star})}_{P^{\star}}]        &\leq  \frac{H^2}{\zeta} \EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\xi\sqrt{\bar C_{\pi(P^{\star} ),P^{\star}  } }\sqrt{\EE_{(s,a)\sim \rho}[\|\phi(s,a)\|^2_{\Sigma^{-1}_n}]} \mid P^{\star},\Zcal}}+2H\delta \\ 
        &\leq  c_1 H^2 \min(d^{1/2},  \bar R)\sqrt{ \bar R }   \sqrt{\frac{d_{\Scal} \ln (1+n) }{n}}\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\sqrt{\bar C_{\pi(P^{\star} ),P^{\star}  } }|\Zcal,P^{\star}} }+2H\delta \\ 
     &\leq  c_1 H^2 \min(d^{1/2},  \bar R)\sqrt{ \bar R }   \sqrt{\frac{d_{\Scal} \ln (1+n) }{n}}\EE_{P^{\star}\sim \beta}\bracks{\sqrt{\bar C_{\pi(P^{\star} ),P^{\star}  } }\EE\bracks{1 |\Zcal,P^{\star}} }+2H\delta \\ 
                &\leq  c_1 H^2 \min(d^{1/2},  \bar R)\sqrt{ \bar R }   \sqrt{\frac{d_{\Scal} \ln (1+n) }{n}}\sqrt{\EE_{P^{\star}\sim \beta}\bracks{\bar C_{\pi(P^{\star} ),P^{\star}  } } }+2H\delta . 
\end{align*}
By taking $\delta=1/n$, the statement is concluded. 


\end{proof}


\begin{proof}[Proof of Corollary \pref{cor:low_rank_bayes}]

We take $L(\pi;\Dcal)$ as $\max(\min(\min_{M\in \Mcal_{\Dcal}}V^{\pi}_{M},H),0)$ in \pref{thm:version}. Then, from the first step in the proof of \pref{thm:version}, conditional on $P^{\star}$, with probability $1-\delta$, $L(\pi;\Dcal)$ satisfies 
\begin{align*}
    L(\pi;\Dcal)\leq V^{\pi}_{P^{\star}},\forall \pi \in \Pi.  
\end{align*}
and 
\begin{align*}
    \EE_{(s,a)\sim \rho}[\|P'(s,a) - P^\star(s,a)  \|^2_1 ]\lesssim \zeta. 
\end{align*}
where $P'=\argmin_{M\in \Mcal_{\Dcal}}V^{\pi(P^{\star})}_{M}$. We denote the above event as $\Zcal$. We have $\mathrm{P}(\Zcal\mid P^{\star})\geq 1-\delta$. 
In addition, from the third step in the proof of \pref{thm:version},  

\begin{align*}
      & \EE[V^{\pi(P^{\star})}_{P^\star} -L(\pi(P^{\star});\Dcal)  ]\leq  \tag{The third step in the proof of \pref{thm:version}} \EE[V^{\pi(P^{\star})}_{P^{\star}}-V^{\pi(P^{\star})}_{P'}] \\
       & \leq H^2\EE_{P^{\star}\sim \beta}[\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|_1 ]] \tag{Simulation lemma, \pref{lem:simulation}}\\
        &\leq H^2\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|_1 ]\mid \Zcal,P^{\star}}P(\Zcal\mid P^{\star})}+\EE_{P^{\star}\sim \beta}[2H(1-P(\Zcal\mid P^{\star}) )]\\
       &\leq H^2\EE_{P^{\star}\sim \beta}\bracks{\EE\bracks{\EE_{(s,a)\sim d^{\pi(P^{\star})}_{P^{\star}}}[\|P'(s,a) - P^\star(s,a)  \|_1 ]\mid \Zcal,P^{\star}}}+2H\delta \\
    &\leq \EE_{P^{\star}\sim \beta}\bracks{\xi^{1/2}|\Acal|H\sqrt{    C_{d_0,P^{\star}}}+|\Acal|H^2\sqrt{\bar C_{\pi(P^{\star}),P^{\star}}\rank(\Sigma_{\rho})}\braces{\frac{\xi}{|\Acal|\min_{(s,a)} \pi_b(a\mid s)}}^{1/2}}+2H\delta \\ 
     &\leq \xi^{1/2}|\Acal|H\sqrt{    C^{\Bayes}_{d_0,\beta}}+|\Acal|H^2\sqrt{\bar C^{\Bayes}_{\beta}\rank(\Sigma_{\rho})}\braces{\frac{\xi}{|\Acal|\min_{(s,a)} \pi_b(a\mid s)}}^{1/2}+2H\delta. 
\end{align*}
\end{proof}




==> some_note.tex <==
\masa{this is just some random thought} 
In Dan Russo's paper (Learning to optimize via posterior sampling, bandit case), from Prop1, they use the decomposition: 
\begin{align*}
   B(T,\pi^{PS})=\EE[\sum_t U_t( A_t)-f_{\theta}(A_t)]+\EE[\sum_t f_{\theta}(A^{*}_t)-U_t(A^{*}_t) ]. 
\end{align*}
($U_t$ can be anything. but let's say this is an upper confidence bound)  Then, we can gain the regret 
\begin{align*}
   B(T,\pi^{PS})& \leq \EE[\sum_t U_t( A_t)-f_{\theta}(A_t)]+\EE[\sum_t f_{\theta}(A^{*}_t)-U_t(A^{*}_t) ]\\
   &=  \EE[\sum_t U_t( A_t)-f_{\theta}(A_t)]+\mathrm{small}=  \EE[\sum_t U_t( A_t)-L_t(A_t)]+small. 
\end{align*}
Then, the regret is obtained as usual. In offline case, what we need to do is 
\begin{align*}
   B(T,\pi^{PS})=\EE[\sum_t L_t( A_t)-f_{\theta}(A_t)]+\EE[\sum_t f_{\theta}(A^{*}_t)-L_t(A^{*}_t) ]. 
\end{align*}
($L_t$ can be anything. but let's say this is a lower confidence bound) Then, we can gain the regret 
\begin{align*}
   B(T,\pi^{PS})& \leq \EE[\sum_t L_t( A_t)-f_{\theta}(A_t)]+\EE[\sum_t f_{\theta}(A^{*}_t)-L_t(A^{*}_t) ]\\
   &= \mathrm{small}+\EE[\sum_t f_{\theta}(A^{*}_t)-L_t(A^{*}_t) ]\leq  \mathrm{small}+\EE[\sum_t U_t(A^{*}_t)-L_t(A^{*}_t) ]. 
\end{align*}


\masa{Just for checking NPG part}

\textbf{Usual Model Based}
\begin{align*}
    V^{\pi^{*}}- V^{\pi_t}& =V^{\pi^{*}} - V^{\pi^{*}}_{\hat P,r-b}+ V^{\pi^{*}}_{\hat P,r-b}-  V^{\hat \pi}\\
    & =V^{\pi^{*}} - V^{\pi^{*}}_{\hat P,r-b}+ V^{\hat \pi}_{\hat P,r-b}-  V^{\hat \pi}\leq V^{\pi^{*}} - V^{\pi^{*}}_{\hat P,r-b}=C_1. 
\end{align*}
We know how to bound $C_1$. 

\textbf{Model based NPG}
\begin{align*}
     V^{\pi^{*}}- V^{\pi_t} &=  V^{\pi^{*}}-  V^{\pi^{*}}_{\hat P,r-b}+V^{\pi^{*}}_{\hat P,r-b}- V^{\pi_t} \\
      &= V^{\pi^{*}}-  V^{\pi^{*}}_{\hat P,r-b} + V^{\pi^{*}}_{\hat P,r-b} - V^{\pi_t}_{\hat P,r-b} +   V^{\pi_t}_{\hat P,r-b} - V^{\pi_t} \leq C_1+ V^{\pi^{*}}_{\hat P,r-b} - V^{\pi_t}_{\hat P,r-b}\\
      &= C_1+ V^{\pi^{*}}_{\hat P,r-b} - V^{\pi_t}_{\hat P,r-b} \\ 
      &= C_1+ H\EE_{s\sim d^{\pi^{*}}_{s_0}}\EE_{a\sim \pi^{*}(\cdot \mid s)}[A^{\pi_t}_{\hat P,r-b }(s,a)]\\ 
      &= C_1+ H\EE_{s\sim d^{\pi^{*}}_{s_0}}\left[\frac{\mathrm{KL}(\pi^{*},\pi^t)- \mathrm{KL}(\pi^{*},\pi^{t-1}) }{\eta }\right]+\mathrm{Error}.
\end{align*}
Here,
\begin{align*}
    \EE\left[\frac{\mathrm{KL}(\pi^{*},\pi^t)- \mathrm{KL}(\pi^{*},\pi^{t-1}) }{\eta }\right]&=\EE_{s\sim d^{\pi^{*}}_{s_0}}\EE_{a\sim \pi^{*}}\left[\log \frac{\pi^t}{\pi^{t-1}}\right]\\
    &=\EE_{s\sim d^{\pi^{*}}_{s_0}}\EE_{a\sim \pi^{*}}[ A^{\pi^{t-1}}(s,a)-\frac{1}{\eta}\log \EE_{a\sim \pi^{t-1}(s)}[\exp(\eta A^{\pi^{t-1}}(s,a)] ] \\ 
    &= \EE_{s\sim d^{\pi^{*}}_{s_0}}\EE_{a\sim \pi^{*}}[ A^{\pi^{t-1}}(s,a)-\eta Z^2 ]. 
\end{align*}





---------------

\section{Detailed analysis}
We assume the model (transition density $P(\cdot\mid \cdot)$) is parametrized by $w\in \mathcal{W}$, where $\mathcal{W}$ is some domain. 
\begin{enumerate}
    \item  Calculate the posterior of $w^{*}$ given $\Dcal$ and denote it by $\rho'(\cdot\mid \cdot)$
    \item Sample a random variable $w$ from $\rho'(\cdot \mid \Dcal)$. 
    \item  Calculate the optimal policy $\pi^w$. 
\end{enumerate}

\begin{theorem}
Suppose $\Dcal$ is the data obtained by the model corresponding to $w\in \mathcal{W}$. Suppose $L(\pi;\Dcal)$ is a function mapping $\Pi$ to $\RR$ depending on $\Dcal$, and 
\begin{align*}
    L(\pi;\Dcal)-V_{w}^{\pi}\leq  0,\quad V_{w^{}}^{\pi}-L(\pi)\leq g(\pi;w),\quad \forall \pi\in \Pi,w\in \mathcal{W}. 
\end{align*}
Then, 
\begin{align*}
 \EE\bracks{  V^{\pi^{w^\star}}_{w^\star}   -  V^{\pi^w}_{w^\star}}\leq  \EE\bracks{ g(\pi^{w^{*}};w^{*})}. 
\end{align*}
\end{theorem}

\begin{proof}
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{Model_based.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

Here, $w^{*}$ is a random variable following the prior $\rho(\cdot)$. $\Dcal$ is the generated data following the model $w^{*}$ and some behavior policy. $w$ follows $\rho'(\cdot \mid \Dcal)$.  This is summarized in the following graphical model. 

The important fact is  
\begin{align*}
    \EE[L(\pi^{w^{*}};\Dcal)]=\EE[\EE[L(\pi^{w^{*}};\Dcal)\mid \Dcal ]]= \EE[\EE[L(\pi^w;\Dcal)\mid \Dcal ]]=\EE[L(\pi^w;\Dcal)].  
\end{align*}

\begin{align*}
 \EE\bracks{  V^{\pi^{w^\star}}_{w^\star}   -  V^{\pi^w}_{w^\star}}&= \EE\bracks{  V^{\pi^{w^\star}}_{w^\star} -L(\pi^{w^{*}};\Dcal)+ L(\pi^{w};\Dcal)- V^{\pi^w}_{w^\star}}\\
  &= \EE\bracks{  V^{\pi^{w^\star}}_{w^\star} -L(\pi^{w^{*}};\Dcal)}+ \EE\bracks{L(\pi^{w};\Dcal)- V^{\pi^w}_{w^\star}}\\
    &= \EE\bracks{  \EE\bracks{V^{\pi^{w^\star}}_{w^\star} -L(\pi^{w^{*}};\Dcal)\mid w^{*}}}+ \EE\bracks{\EE\bracks{L(\pi^{w};\Dcal)- V^{\pi^w}_{w^\star}\mid w^{*}}}\\
    &\leq  \EE\bracks{ g(\pi^{w^{*}};w^{*})}. 
\end{align*}

\end{proof} 

We analyze the following algorithm. Here, $\Dcal=\{\Dcal_1,\cdots,\Dcal_T\}$, and $\bar \Dcal_t=\{\Dcal_1,\cdots,\Dcal_t\}$.  

Initialize $\pi^1$; For $t = 1$ to $T$, repeat:
\begin{enumerate}
\item Calculate the posterior distribution of $w^{*}$ given $\Dcal_t$ and denote it by $\rho_t(\cdot\mid \cdot)$
\item Sample a model $w_t \sim \rho_t(\cdot | \bar \Dcal_t)$ 
\item Compute advantage value of $\pi^t$ under $w_t$, denoted as $A^{\pi^t}_{w_t}(s,a)$; 
\item Perform soft policy improvement $\pi^{t+1}(\cdot | s) \propto \pi^t(\cdot \mid s)\exp\left( \eta A^{\pi^t}_{w_t}(s,\cdot) \right)$.
\end{enumerate}

We can use the whole history $\Dcal$. 

\begin{theorem} 
Suppose $L_t(\pi;\bar \Dcal_t)$ is a function mapping $\Pi$ to $\RR$ depending on $\Dcal_t$. When $\Dcal_t$ is the data generated from $w$, we assume 
\begin{align*}
    L_t(\pi;\bar \Dcal_t)-V_{w}(\pi)\leq  0,\quad V_{w}(\pi)-L_t(\pi;\bar \Dcal_t)\leq g_t(\pi; w),\quad \forall \pi\in \Pi,w\in \mathcal{W}. 
\end{align*}
Suppose $\eta\leq 1/Z, A^{\pi}_{w}(s,a)\leq Z\,(\forall \pi \in \Pi,w\in \mathcal{W})$. Then, 

\begin{align*}
\min_{t\leq T}  \EE\bracks{  V^{\pi^{w^\star}}_{w^\star}   -  V^{\pi^t}_{w^\star}}\leq \braces{\min_{t\leq T}  \EE\bracks{g_t(\pi^{w^{*}};w^{*}) }}+\frac{2Z\sqrt{\log |\Acal|}}{\sqrt{T}}.  
\end{align*}

\end{theorem}

We often use the following relation.  Let $X,Y,X'$ be random variables. 
Then, given a function $f$ over $X,Y,Z$, when the pdf of $X$ given $Y,Z$ and the pdf of $X'$ given $Y,Z$ are the same, we have
\begin{align*}
    \EE[f(X,Y,Z)]=\EE[\EE[f(X,Y,Z)\mid Y,Z)]]=\EE[\EE[f(X',Y,Z)\mid Y)]]=\EE[f(X',Y,Z)]. 
\end{align*} 
However, we need to be careful even if the pdf of $X$ given $Y$ and the pdd of $X'$ given $Y$ are the same, we cannot exchange $X$ and $X'$. 
Hereafter, given any random variables $X,Y$, we denote its pdf as $P(X\mid Y)$. 

\begin{proof}
We prove the sample splitting version. But, this proof can be directly applied to the case when we use the whole data by just changing $\Dcal_t$ to $\Dcal$. See several remarks in the proof to validate the swapping of some random variables. 

Here, $w^{*}\sim \rho(\cdot),\Dcal_t \sim  d(\cdot \mid w^{*})$. Then, by denoting the posterior distribution of $w^{*}$ given $\bar \Dcal_t$ as $\rho_t(\cdot\mid \cdot)$, then $w_t\sim \rho_t(\cdot \mid \bar \Dcal_t)$. Besides, we define a dummy random variable  
$w'_t\sim \rho_t(\cdot \mid \bar \Dcal_t)$. $w_t$ and $w'_t $ are conditionally independent given $\Dcal_t$. The relation of random variables is described in the following graphical model. 
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{NPG.pdf}
    \caption{Use the historical data up to $t$}
    \label{fig:my_label}
\end{figure}
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\linewidth]{NPG_whole.pdf}
    \caption{Use the whole data }
    \label{fig:my_label}
\end{figure}

Then, we have 
\begin{align*}
  \EE\bracks{  V^{\pi^{w^\star}}_{w^\star}   -  V^{\pi^t}_{w^\star}}&=\EE\bracks{ V^{\pi^{w^\star}}_{w^\star} -L_t(\pi^{w^{*}};\bar \Dcal_t)+  L_t(\pi^{w^{*}};\bar \Dcal_t)- V^{\pi^t}_{w^\star} } \\ 
  &=\EE\bracks{ V^{\pi^{w^\star}}_{w^\star} -L_t(\pi^{w^{*}};\bar \Dcal_t)+  \EE[L_t(\pi^{w^{*}};\bar \Dcal_t)\mid \bar \Dcal_t]- V^{\pi^t}_{w^\star} } \\ 
    &=\EE\bracks{ V^{\pi^{w^\star}}_{w^\star} -L_t(\pi^{w^{*}};\bar \Dcal_t)+  \EE[L_t(\pi^{w'_t};\bar \Dcal_t)\mid \bar \Dcal_t]- V^{\pi^t}_{w^\star} } \\ 
  &= \EE\bracks{ V^{\pi^{w^\star}}_{w^\star} -L_t(\pi^{w^{*}};\bar \Dcal_t)+  L_t(\pi^{w'_t};\bar \Dcal_t)- V^{\pi^t}_{w^\star} }\\
    &\leq  \EE\bracks{g_t(\pi^{w^{*}};w^{*}) }+ \EE\bracks{L_t(\pi^{w'_t};\bar \Dcal_t)- V^{\pi^t}_{w^\star} }. \tag{Assumption} 
\end{align*}
From the second line to the third line, we use $P(w^{*}\mid \bar \Dcal_t)=\rho_t(w^{*}\mid \bar \Dcal_t)$, $P(w'_t\mid \bar \Dcal_t)=\rho_t(w'_t\mid \bar \Dcal_t)$. 


Besides, from the assumption, 
\begin{align*}
   \EE\bracks{L_t(\pi^{w'_t};\bar \Dcal_t)}=  \EE\bracks{\EE[L_t(\pi^{w'_t};\bar \Dcal_t)\mid w^{*}]}\leq \EE\bracks{\EE\bracks{V_{w^{*}}^{\pi^{w'_t}} \mid w^{*}}}=\EE\bracks{V_{w^{*}}^{\pi^{w'_t}} }. 
\end{align*}
Thus, 
\begin{align*}
   \EE\bracks{L_t(\pi^{w_t};\bar \Dcal_t)- V^{\pi^t}_{w^\star} }&\leq   \EE\bracks{V_{w^{*}}^{\pi^{w'_t}} - V^{\pi^t}_{w^\star} }\\
   &=\frac{1}{1-\gamma}\EE[ \EE_{(s,a) \sim d_{w^{*}}^{\pi^{w'_t}} }[A^{\pi_t}_{w^{*}}(s,a)] ] \tag{Performance difference lemma}\\
    &=\frac{1}{1-\gamma}\EE[ \EE[\EE_{(s,a) \sim d_{w^{*}}^{\pi^{w'_t}} }[A^{\pi_t}_{w^{*}}(s,a)] \mid \bar \Dcal_{t},\pi_t,w'_t] ] \tag{Tower property}\\
 &=\frac{1}{1-\gamma}\EE[ \EE[\EE_{(s,a) \sim d_{w_t}^{\pi^{w'_t}} }[A^{\pi_t}_{w_{t}}(s,a)]\mid \bar \Dcal_{t},\pi_t,w'_t] ] \\ 
  &=\frac{1}{1-\gamma}\EE[\EE_{(s,a) \sim d_{w_t}^{\pi^{w'_t}} }[A^{\pi_t}_{w_{t}}(s,a)]]. \tag{Tower property}
\end{align*}   
From the third line to the fourth line, we use
\begin{align*}
    P(w^{*}\mid \bar \Dcal_{t},\pi_t,w'_t)=   P(w^{*}\mid \bar \Dcal_{t})=\rho_{t}(w^{*} \mid  \bar \Dcal_{t}),\quad     P(w_t \mid \bar \Dcal_{t},\pi_t,w'_t)= \rho_{t}(w_t \mid  \bar \Dcal_{t}). 
\end{align*}

 --------------
 
When we use the whole history,  
 \begin{align*}
    P(w^{*}\mid \bar \Dcal,\pi_t,w'_t)=   P(w^{*}\mid \bar \Dcal)=\rho_{t}(w^{*} \mid  \bar \Dcal),\quad     P(w_t \mid \bar \Dcal,\pi_t,w'_t)= \rho_{t}(w_t \mid  \bar \Dcal). 
\end{align*}

 ----------
 
Here, we have 
\begin{align*}
    \EE_{(s) \sim d_{w_t}^{\pi^{w'_t}} }\bracks{\frac{KL( \pi^{w'_t},\pi_{t+1})(s)-KL(\pi^{w'_t},\pi_t)(s)}{\eta}}&= \EE_{(s) \sim d_{w_t}^{\pi^{w'_t}},a\sim \pi^{w'_t} }\bracks{\log\frac{\pi^{t+1}(a\mid s)}{\pi^t(a\mid s)} }\\ 
    &=\EE_{(s) \sim d_{w_t}^{\pi^{w'_t}},a\sim \pi^{w'_t} }\bracks{A^{\pi^t}_{w_t}(s,a)-\frac{1}{\eta}\log\EE_{a\sim \pi^{t}}[\exp(\eta  A^{\pi^t}_{w_t}(s,a)] } \\ 
    &\geq \EE_{(s) \sim d_{w_t}^{\pi^{w'_t}},a\sim \pi^{w'_t} }\bracks{A^{\pi^t}_{w_t}(s,a)}-\eta Z^2 . 
\end{align*}
From the second line to third line, we use the following 
\begin{align*}
    \log\EE_{a\sim \pi^{t}}[\exp(\eta  A^{\pi^t}_{w_t}(s,a)]& \leq  \log\braces{\EE_{a\sim \pi^{t}}[1+\eta  A^{\pi^t}_{w_t}(s,a)+\{\eta  A^{\pi^t}_{w_t}(s,a)\}^2] } \tag{$\eta\leq 1/Z,\exp(x)\leq 1+x+x^2 (x\leq 1)$}\\
    & \leq \log\braces{\EE_{a\sim \pi^{t}}[1+\eta^2 Z^2 ] }\leq \eta^2Z^2 . 
\end{align*}
   
Then, 
\begin{align*}
     \EE\bracks{L(\pi^{w_t};\Dcal)- V^{\pi^t}_{w^\star} }   &=\frac{1}{1-\gamma}\EE[\EE_{(s,a) \sim d_{w_t}^{\pi^{w'_t}} }[\EE[A^{\pi_t}_{w_{t}}(s,a) ]]\\
      &\leq \frac{1}{1-\gamma}\EE\bracks{\EE_{(s) \sim d_{w_t}^{\pi^{w'_t}} }\bracks{\eta Z^2 +\frac{KL( \pi^{w'_t},\pi_{t+1})(s)-KL(\pi^{w'_t},\pi_t)(s)}{\eta}} }\\
     &=\frac{1}{1-\gamma}\EE\bracks{\EE\bracks{\EE_{(s) \sim d_{w_t}^{\pi^{w'_t}} }\bracks{\eta Z^2 +\frac{KL( \pi^{w'_t},\pi_{t+1})(s)-KL(\pi^{w'_t},\pi_t)(s)}{\eta}} \mid \bar \Dcal_t,\pi_{t+1},\pi_t}}\\ 
    &=\frac{1}{1-\gamma}\EE\bracks{\EE\bracks{\EE_{(s) \sim d_{w_t}^{\pi^{w^{*}}} }\bracks{\eta Z^2 +\frac{KL( \pi^{w^{*}},\pi_{t+1})(s)-KL(\pi^{w^{*}},\pi_t)(s)}{\eta}} \mid \bar \Dcal_t,\pi_{t+1},\pi_t}}\\  
    &=\frac{1}{1-\gamma}\EE\bracks{\EE_{(s) \sim d_{w_t}^{\pi^{w^{*}}} }\bracks{\eta Z^2 +\frac{KL( \pi^{w^{*}},\pi_{t+1})(s)-KL(\pi^{w^{*}},\pi_t)(s)}{\eta}}}\\  
\end{align*}

From the third line to the fourth line, we use 
\begin{align*}
    P(w'_t\mid \bar \Dcal_t,\pi_{t+1},\pi_t)=    P(w'_t\mid \bar \Dcal_t)=\rho_t(w'_t\mid \bar \Dcal_t),\quad P(w^{*}\mid  \bar \Dcal_t,\pi_{t+1},\pi_t)= \rho_t(w^{*} \mid \bar \Dcal_t). 
\end{align*}

---------------

When we use the whole history, from the third line to the fourth line, we use 
\begin{align*}
    P(w'_t\mid \bar \Dcal,\pi_{t+1},\pi_t)=    P(w'_t\mid \bar \Dcal)=\rho_t(w'_t\mid \bar \Dcal),\quad P(w^{*}\mid  \bar \Dcal,\pi_{t+1},\pi_t)= \rho_t(w^{*} \mid \bar \Dcal). 
\end{align*}

----------------

Finally, 
\begin{align*}
     & \min_{t\leq T}\EE\bracks{  V^{\pi^{w^\star}}_{w^\star}   -  V^{\pi^t}_{w^\star}}\\
     &\leq \braces{\min_{t\leq T} \EE\bracks{g_t(\pi^{w^{*}};w^{*}) }}+\frac{1}{T}\sum_{t=1}^T \EE\bracks{L(\pi^{w'_t};\bar \Dcal_t)- V^{\pi^t}_{w^\star} }\\
     &\leq \braces{\min_{t\leq T} \EE\bracks{g_t(\pi^{w^{*}};w^{*}) }}+ \frac{1}{1-\gamma}\braces{\eta Z^2+\frac{1}{T}\EE\bracks{\EE_{(s) \sim d_{w_t}^{\pi^{w^{*}}} }\bracks{\frac{KL( \pi^{w^{*}},\pi_{T+1})(s)-KL(\pi^{w^{*}},\pi_1)(s)}{\eta}}}}\\
     &\leq \braces{\min_{t\leq T} \EE\bracks{g_t(\pi^{w^{*}};w^{*}) }}+\frac{1}{1-\gamma}\braces{\eta Z^2+\frac{\log |\Acal|}{\eta T} }\\
     & \leq \braces{\min_{t\leq T} \EE\bracks{g_t(\pi^{w^{*}};w^{*}) }}+2Z\sqrt{\frac{\log |\Acal|}{T}}. 
\end{align*}

\end{proof}
